Global Convergence of Policy Gradient Methods to (Almost) Locally Optimal Policies

Policy gradient (PG) methods are a widely used reinforcement learning methodology in many applications such as video games, autonomous driving, and robotics. In spite of its empirical success, a rigorous understanding of the global convergence of PG methods is lacking in the literature. In this work, we close the gap by viewing PG methods from a nonconvex optimization perspective. In particular, we propose a new variant of PG methods for infinite-horizon problems that uses a random rollout horizon for the Monte-Carlo estimation of the policy gradient. This method then yields an unbiased estimate of the policy gradient with bounded variance, which enables the tools from nonconvex optimization to be applied to establish global convergence. Employing this perspective, we first recover the convergence results with rates to the stationary-point policies in the literature. More interestingly, motivated by advances in nonconvex optimization, we modify the proposed PG method by introducing periodically enlarged stepsizes. The modified algorithm is shown to escape saddle points under mild assumptions on the reward and the policy parameterization. Under a further strict saddle points assumption, this result establishes convergence to essentially locally-optimal policies of the underlying problem, and thus bridges the gap in existing literature on the convergence of PG methods. Results from experiments on the inverted pendulum are then provided to corroborate our theory, namely, by slightly reshaping the reward function to satisfy our assumption, unfavorable saddle points can be avoided and better limit points can be attained. Intriguingly, this empirical finding justifies the benefit of reward-reshaping from a nonconvex optimization perspective.

==> Introduction__1_.tex <==
%!TEX root = Policy_Grad.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S  E  C T  I  O  N%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}  
% 
%In reinforcement learning (RL) \cite{sutton2017reinforcement,bertsekas2005dynamic}, an autonomous agent moves through a state space  and seeks to learn a policy  which maps states to a probability distribution over actions to maximize a long-term accumulation of rewards. When the agent selects a given action at a particular state, a reward is revealed and a random transition to a new state occurs according to a probability density that only depends on the current state and action, i.e., state transitions are Markovian. In this way, the agent must glean the merit of different actions by interacting with the environment.
%
%Two dominant approaches to reinforcement learning have emerged: those based on optimizing the value function directly, referred to as  ``direct policy search'', and those based on solving the Bellman fixed point equations \cite{bellman57a}. The goal of this work is to rigorously understand the former approach: direct policy search, specifically policy gradient methods \cite{sutton2000policy}. Policy search has gained traction recently due to its ability to scale gracefully to large and even continuous spaces \cite{silver2014deterministic,schulman2015trust} and incorporate deep networks \cite{lillicrap2015continuous,mnih2016asynchronous}. 
%
%Despite the increasing prevalence of policy gradient methods, their global convergence in the discounted infinite-horizon setting,  which is conventional in dynamic programming \cite{bertsekas2005dynamic},  is not well understood . This gap  stems firstly  from the fact that obtaining unbiased estimates of the policy gradient through sampling is often elusive. 
%Specifically, following the Policy Gradient Theorem \cite{sutton2000policy},
%%yields the fact that the policy gradient contains two distinct factors: (1) the score function, i.e., the gradient of the logarithm of the policy, and (2) the action-value (or $Q$) function induced by a particular policy, both evaluated at a state-action pair drawn from an ergodic distribution of the Markov chain under the policy.  
%obtaining an unbiased estimate of the policy gradient requires two significant conditions to hold: (1) the state-action pair is drawn from the discounted state-action occupancy measure  of the Markov chain under the policy; (2) the estimate of the action-value (or $Q$) function induced by the  policy is unbiased.   
%The gap also results from the fact that  the value function to be maximized in RL is in general \emph{nonconvex} with respect to the policy parameter \cite{fazel2018global,bhandari2019global}. It is worth mentioning that although the recent work \cite{fazel2018global}, and the concurrent work \cite{bhandari2019global} have identified several special RL settings where the stationary-points align with the global optimum, our focus is on a broader RL regime where the  nonconvexity is general such that solving the problem can be  NP-hard.  
% 
%%and as a result  one must quantify the stochastic descent directional error. 
%
%% (``the double sampling problem"). 
%%While the former factor may be estimated using sampling, the later depends on the policy parameters, which change across iterations. 
%
%%\kznote{Probably we may want to not use the term "double sampling". In RL, double sampling is reserved for the case when expected value of the product does not equal the product of two expected values in policy evaluation. In policy gradient method, what we have is just a "double-loop" expectation. }
%
%
%Monte-Carlo rollout, i.e., having the agent randomly explore the state-action space and accumulate rewards, up to some time horizon, may be used to obtain unbiased estimates of the action-value when one restricts focus to \emph{episodic} reinforcement learning. However, this finite horizon rollout will be biased with respect to an infinite-horizon discounted value function. 
%%This bias issue has led most analyses to focus on asymptotic behavior by invoking connections to dynamical systems \cite{borkar2000ode,borkar2008stochastic}. 
%%, although some efforts towards finite sample analysis of the infinite-horizon case have appeared recently for linear systems \cite{fazel2018global}. 
%To handle this bias, we employ in this work  random geometric time rollout horizons, a technique first formulated in \cite{santi2018stochastic}. This allows us to obtain unbiased estimates of the $Q$ function, using only rollouts with finite horizons. Moreover, the random rollout horizon also gives rise to an unbiased sampling of the state-action pair from the discounted  occupancy measure.  With these two challenges addressed,  an unbiased estimate of the policy gradient can be  obtained, which allows us to strengthen the link between the policy gradient method and the classical stochastic programming \cite{shapiro2009lectures}. We refer to our algorithm as \emph{random-horizon}  policy gradient (RPG), to emphasize that the horizon of the Monte-Carlo rollout is random. 
%%We refer to the resulting variant of policy gradient method as \emph{R3INFORCE}, since it is established upon the Monte-Carlo rollout of trajectories  as REINFORCE  \cite{sutton2000policy}, but with \emph{random} rollout horizons.
%
%%\kznote{I think we should not say "nothing more than", since our algorithm, although is based on Monte-Carlo rollout, is still different from the actual REINFORCE. In particular, we estimate $Q$-value and score function for a specific $(s,a)$, while REINFORCE evaluate the rollout return and the score function "along the whole trajectory".}
%
%Leveraging this connection, we are able to address a noticeably open issue in policy {gradient methods}: a technical understanding of the effect of the policy parameterization on both the limiting and finite-iteration algorithm behaviors. In particular, it is well known  in nonconvex optimization that with only first-order information and no additional hypothesis, convergence to a stationary point {with zero gradient-norm }is the best one may hope to achieve \cite{wright1999numerical}. 
%{However, in some asymptotic analyses for policy gradient methods with function approximation \cite{pirotta2015policy}, or their  variant, actor-critic algorithms \cite{bhatnagar2008incremental,bhatnagar2009natural,bhatnagar2010actor,chow2017risk}, it was claimed that the limit points of the algorithms starting from any initialization  constitute the \emph{locally-optimal policies}, i.e., the algorithms enjoy global  convergence  to the local-optima.  
%However, by the theory of stochastic approximation \cite{borkar2008stochastic}, such a claim can only be made locally, i.e., 
%the local-optimality can only  be obtained if the algorithm starts around a local minima,   under the assumption that a \emph{strict} Lyapunov function exists. Therefore, \emph{global}  convergence of PG methods to the \emph{actual locally-optimal }policies, though claimed in words in some literature, is still an open question.  
%Another line of  theoretical studies  of policy gradient methods only focuses on showing the one-step policy improvement  \cite{pirotta2013adaptive,pirotta2015policy,papini2017adaptive}, by choosing appropriate stepsizes and/or batch data sizes. Such one-step result still does not imply any global convergence result.    
%In summary, the misuse of the term \emph{locally-optimal policy} and the lack of studying global convergence property of PG methods  motivate us to further investigate this problem from a nonconvex optimization perspective. Thanks to  the analytical tools from optimization, we are able to first recover the asymptotic convergence, and then provide the convergence rate, to \emph{stationary-point} policies. 
%} 
%
% %
%%\kznote{I  think the colored ones have some issues, and indeed need to be revised. First, to my knowledge there is no work that use ODE (or dynamical systems theory) to analyze "policy gradient" method, they use ODE to analyze actor-critic. Thus, we should say that there exists no "systematic" (or "general") analysis for PG. Second, the "existence  of Lyapunov function", the argument is not correct. For optimization problem, the Lyapunov function always exists, and is just the value function (in a local area), no matter it is nonconvex or not. But this theory only dictates "local" convergence property, this should be something we want to emphasize, not the "existence" or the "convex" parts. Third, we may want to mention  that most of the existing analysis for PG are only : i) providing "one-step policy improvement"; ii) misuse the term "local optimal policy" that the algorithm may converge to (it is in fact just the "stationary point" that "the best one can hope for"). }
%
%
%Heartened by this connection between nonconvex optimization and policy search, we then  tackle a related question: what implications do recent advances in nonconvex optimization ( \cite{jin2017escape,daneshmand2018escaping}) that escape saddle points have on policy gradient methods? In  \S\ref{sec:conv_second_stationary_point}, we identify structural properties of reinforcement learning that can be exploited to mitigate nonconvexity when suitable hypotheses are made on the policy parameterization and reward. Specifically, when the reward is positive and bounded, and the policy parameterization is \emph{regular}, i.e., its Fisher  information is positive definite (a conventional assumption in RL \cite{kakade2002natural}), the correlated negative curvature condition of \cite{daneshmand2018escaping} holds. Thus, we can establish the result that policy gradient methods can escape saddle points and converge to \emph{second-order} stationary solutions, as well as to discern rates when a \emph{periodically enlarged stepsize} strategy is employed. We call the resulting method Modified RPG (MRPG). The positivity requirement on the reward for this setting further motivates use of a modified update where we substitute the $Q$ function by a $Q$ function minus a baseline, for the purpose of variance reduction. {The modified update that uses baselines is also shown to converge to second-order stationary-point polices. }
%%\kznote{What did you mean by "the same convergence guarantees"? This is convergence to 2nd-order stationary point, right? Also, should we have a name for this algorithm, say, Modified R3INFORCE? Currently in the simulation figures, we can the algorithms \emph{RPG and MRPG}.}

In reinforcement learning (RL) \cite{sutton2017reinforcement,bertsekas2005dynamic}, an autonomous agent moves through a state space  and seeks to learn a policy  which maps states to a probability distribution over actions to maximize a long-term accumulation of rewards. When the agent selects a given action at a particular state, a reward is revealed and a random transition to a new state occurs according to a probability density that only depends on the current state and action, i.e., state transitions are Markovian. {This evolution process is usually modeled as a Markov decision process (MDP). } Under this setting, the agent must evaluate the merit of different actions by interacting with the environment. 
Two dominant approaches to reinforcement learning have emerged: those based on optimizing {the accumulated reward  directly from the policy space}, referred to as  ``direct policy search'', and those based on {finding the value function by} 
solving the Bellman fixed point equations \cite{bellman57a}. The goal of this work is to rigorously understand the former approach of direct policy search, specifically policy gradient (PG) methods \cite{sutton2000policy}. Policy search has gained traction recently, thanks to  its ability to scale gracefully to large and even continuous spaces  \cite{silver2014deterministic,schulman2015trust} and to incorporate deep networks {as function approximators  }\cite{lillicrap2015continuous,mnih2016asynchronous}. 

Despite the increasing prevalence of policy gradient methods, their global convergence in the infinite-horizon discounted setting,  which is conventional in dynamic programming \cite{bertsekas2005dynamic},  is not yet well understood. This gap  stems firstly  from the fact that obtaining unbiased estimates of the policy gradient through sampling is often elusive. 
Specifically, following the Policy Gradient Theorem \cite{sutton2000policy},
%yields the fact that the policy gradient contains two distinct factors: (1) the score function, i.e., the gradient of the logarithm of the policy, and (2) the action-value (or $Q$) function induced by a particular policy, both evaluated at a state-action pair drawn from an ergodic distribution of the Markov chain under the policy. 
obtaining an unbiased estimate of the policy gradient requires two significant conditions to hold: (i) the state-action pair is drawn from the discounted state-action occupancy measure  of the Markov chain under the policy; (ii) the estimate of the action-value (or $Q$) function induced by the  policy is unbiased.   
This gap also results from the fact that  the value function to be maximized in RL is in general \emph{nonconvex} with respect to the policy parameter \cite{fazel2018global,zhang2019policy,bhandari2019global,liu2019neural,agarwal2019optimality}. 
In the same vein as our work, there is a surging interest in studying the global convergence of PG methods, see the recent work  \cite{fazel2018global,zhang2019policy,bu2019lqr}, and concurrent work \cite{bhandari2019global,liu2019neural,agarwal2019optimality}. However, it  is worth mentioning that orthogonal to our work, these work considered convergence to the \emph{global optimum} in several \emph{special} 	RL settings, e.g., linear quadratic setting \cite{fazel2018global,bu2019lqr}, tabular setting \cite{bhandari2019global,agarwal2019optimality}, or the setting with function approximation but the approximation error can be quantified \cite{agarwal2019optimality}. 
%although the recent work \cite{fazel2018global}, and the concurrent work \cite{bhandari2019global,liu2019neural,agarwal2019optimality} have identified several special RL problems with  certain policy parameterization can achieve global optima, 
In contrast, our focus is on a broader RL regime where the  nonconvexity is general, so that solving the problem can be  NP-hard.    

% (``the double sampling problem"). 
%While the former factor may be estimated using sampling, the later depends on the policy parameters, which change across iterations. 

%\kznote{Probably we may want to not use the term "double sampling". In RL, double sampling is reserved for the case when expected value of the product does not equal the product of two expected values in policy evaluation. In policy gradient method, what we have is just a "double-loop" expectation. }


{
When one restricts the  focus to \emph{episodic} reinforcement learning, 
Monte-Carlo rollout may be used to obtain \emph{unbiased} estimates of the Q-function. In particular, the  rollout   simulates the MDP under certain policy up to a finite time horizon, and then collects  the rewards and state-action histories along the trajectory. }
 However, this finite-horizon rollout, {though generally used in practice,} is known to introduce bias in estimating an \emph{infinite-horizon}  discounted value function. 
Such  a bias in estimating the policy gradient for infinite-horizon problems has been identified in the earlier  work \cite{baxter2001infinite,bartlett2011experiments}, both analytically and empirically.  
%This bias issue has led most analyses to focus on \emph{asymptotic} behavior by invoking connections to dynamical systems \cite{borkar2000ode,borkar2008stochastic}, while some recent efforts towards \emph{finite sample analysis} of the infinite-horizon case have appeared recently for linear quadratic problems only, a special case of general MDPs.  \cite{fazel2018global}. 
%{In fact, such a bias in estimating the policy gradient for infinite-horizon problems has been identified in the earlier  work \cite{baxter2001infinite,bartlett2011experiments}, both analytically and empirically.  }
To address this bias issue, we employ in this work  random geometric time rollout horizons, a technique first proposed in \cite{santi2018stochastic}. This rollout procedure  allows us to obtain unbiased estimates of the $Q$ function, using only rollouts of finite horizons. Moreover, the random rollout horizon also creates an unbiased sampling of the state-action pair from the discounted  occupancy measure \cite{sutton2000policy}.  With these two challenges addressed,  the policy gradient can be estimated unbiasedly. Consequently,    the policy gradient methods  can be more naturally connected to  the classical stochastic programming algorithms  \cite{shapiro2009lectures}, {where the unbiasedness of the stochastic gradient   is a critical assumption}. We refer to our algorithm as \emph{random-horizon}  policy gradient (RPG), to emphasize that the finite horizon of the Monte-Carlo rollout is random. 
%We refer to the resulting variant of policy gradient method as \emph{R3INFORCE}, since it is established upon the Monte-Carlo rollout of trajectories  as REINFORCE  \cite{sutton2000policy}, but with \emph{random} rollout horizons.

%\kznote{I think we should not say "nothing more than", since our algorithm, although is based on Monte-Carlo rollout, is still different from the actual REINFORCE. In particular, we estimate $Q$-value and score function for a specific $(s,a)$, while REINFORCE evaluate the rollout return and the score function "along the whole trajectory".}


Leveraging this connection, we are able to address a noticeably open issue in policy {gradient methods}: a technical understanding of the effect of the policy parameterization on both the limiting and finite-iteration algorithm behaviors. In particular, it is well known  in nonconvex optimization that with only first-order information and no additional hypothesis, convergence to a stationary point {with zero gradient-norm }is the best one may hope to achieve \cite{wright1999numerical}.  
Indeed, this is the type of points that most current PG methods are guaranteed to converge to, as pointed out by  \cite{agarwal2019optimality}.  
{However, in some asymptotic analyses for policy gradient methods with function approximation \cite{pirotta2015policy}, or their  variant, actor-critic algorithms \cite{bhatnagar2008incremental,bhatnagar2009natural,bhatnagar2010actor,chow2017risk}, it was claimed that the limit points of the algorithms starting from any initialization  constitute the \emph{locally-optimal policies}, i.e., the algorithms enjoy global  convergence  to the local-optima.  
However, by the theory of stochastic approximation \cite{borkar2008stochastic}, such a claim can only be made locally, i.e., 
the local-optimality can only  be obtained if the algorithm starts around a local minima,   under the assumption that a \emph{strict} Lyapunov function exists. Therefore, \emph{global}  convergence of PG methods to the \emph{actual locally-optimal }policies, though claimed in words in some literature, is still an open question.  
Another line of  theoretical studies  of policy gradient methods only focuses on showing the one-step policy improvement \cite{pirotta2013adaptive,pirotta2015policy,papini2017adaptive}, by choosing appropriate stepsizes and/or batch data sizes. Such one-step result still does not imply any global convergence result.    
In summary, the misuse of the term \emph{locally-optimal policy} and the lack of studying global convergence property of PG methods  motivate us to further investigate this problem from a nonconvex optimization perspective. Thanks to  the analytical tools from optimization, we are able to first recover the asymptotic convergence, and then provide the convergence rate, to \emph{stationary-point} policies. 
}

%\issue{I do not fully understand this argument, and not sure if this is accurate!! Borkar never claimed  convergence to ``local policy''. I tried to re-write it in the previous paragraph. }  However, numerous analyses of policy gradient methods claim global convergence to local minimizers by invoking dynamical systems theory \cite{borkar2000ode,borkar2008stochastic}.  The validity of this analysis hinges on the existence of a strict Lyapunov function; however, for \edit{policy gradient methods}, unless additional structure is present, only a \emph{nonstrict} Lyapunov function can be defined, and hence \emph{stationarity} would be the valid limit of the  policy gradient method. Moreover, without a global descent property, only local convergence may be established. In summary, existing analyses for policy search are limited in that they (i) provide only one-step policy improvement; and ii) misuse the term \emph{local-optimal policy} as the algorithm limit, when in fact it is a stationary point.
%In  \S\ref{sec:alg}, we close these gaps by establishing a link between policy search and submartingales \cite{durrett2010probability}, which allows us to provide a unified asymptotic analysis, and consequently yields the first finite-iteration analysis as well as constant stepsize behavior.
%\issue{ See if my previous paragraph can replace this one.}
 
 %
%\kznote{I  think the colored ones have some issues, and indeed need to be revised. First, to my knowledge there is no work that use ODE (or dynamical systems theory) to analyze "policy gradient" method, they use ODE to analyze actor-critic. Thus, we should say that there exists no "systematic" (or "general") analysis for PG. Second, the "existence  of Lyapunov function", the argument is not correct. For optimization problem, the Lyapunov function always exists, and is just the value function (in a local area), no matter it is nonconvex or not. But this theory only dictates "local" convergence property, this should be something we want to emphasize, not the "existence" or the "convex" parts. Third, we may want to mention  that most of the existing analysis for PG are only : i) providing "one-step policy improvement"; ii) misuse the term "local optimal policy" that the algorithm may converge to (it is in fact just the "stationary point" that "the best one can hope for"). }


Encouraged by this connection between nonconvex optimization and policy search, we then  tackle a related question: what implications do recent algorithms   that can escape saddle points for nonconvex problems (\cite{jin2017escape,daneshmand2018escaping}) have on policy gradient methods in RL? To answer this question,   we identify several  structural properties of  RL problems   that can be exploited to mitigate the underlying  nonconvexity, {which rely on  some  key assumptions on the } policy parameterization and reward. Specifically, {the reward needs to be bounded and {either strictly positive or negative}, and the policy parameterization need to be  \emph{regular}, i.e., its Fisher  information {matrix} is positive definite (a conventional assumption in RL \cite{kakade2002natural}).} {Under these mild  conditions,} we can establish  that policy gradient methods can escape saddle points and converge to  \emph{second-order} stationary points {with high probability},  when a \emph{periodically enlarged stepsize} strategy is employed. We {refer to the resulting method as Modified RPG (MRPG)}. 
{Nevertheless, the strict positivity/{negativity} of reward function may amplify the variance of the  gradient estimate, compared to the setting  that has reward values with both signs but of smaller magnitude. This increased variance  can be alleviated by introducing a \emph{baseline} in the gradient estimate, as advocated  by  existing  work  \cite{greensmith2004variance,peters2006policy,bhatnagar2008incremental}. Therefore, we propose two further modified updates that include the baselines, both  shown to converge to second-order stationary points  as well. 


\vspace{6pt}
\noindent \textbf{Main Contribution:} The main contribution of the present work is three-fold: i) we propose a series of random-horizon PG methods that unbiasedly estimate the true policy gradient for \emph{infinite-horizon discounted}  MDPs, which facilitates the use of analytical tools from nonconvex optimization to establish their convergence to \emph{stationary-point} policies; ii) by virtue of such a  connection of PG methods and nonconvex optimization, we propose   modified RPG methods with periodically enlarged stepsizes, with guaranteed convergence  to actual \emph{locally-optimal policies} under mild conditions on the reward functions and parametrization  of the policies; iii) we connect  the condition on the reward function to the  reward-reshaping technique advocated in empirical RL studies, justifying its benefit, both analytically and empirically, from a nonconvex optimization perspective. Additionally, we believe such a perspective opens the door to exploiting more advancements in nonconvex optimization to improve the convergence properties of policy gradient methods in RL.  
}
%\issue{Check this out, may be further simplified.}
%\issue{The strict positivity/\edit{negativity} requirement on the reward for this setting further motivates use of a modified update where we substitute the $Q$ function by a $Q$ function minus a baseline, for the purpose of variance reduction. The modified update that uses baselines is also shown to converge to second-order stationary points. }

%\kznote{What did you mean by "the same convergence guarantees"? This is convergence to 2nd-order stationary point, right? Also, should we have a name for this algorithm, say, Modified R3INFORCE? Currently in the simulation figures, we can the algorithms \emph{RPG and MRPG}.}

%


%
The rest of the paper is organized as follows. In  \S\ref{sec:prob}, we clarify the problem setting of reinforcement learning and the technicalities of Markov Decision Processes. In  \S\ref{sec:alg} we develop the policy gradient method using random geometric Monte-Carlo rollout horizons,  i.e., the RPG method. Further, we establish both its limiting (Theorem \ref{thm:alg1_as_conv}) and finite-sample  (Theorem \ref{thm:alg1_conv_rate} and Corollary \ref{coro:alg1_conv_rate_const_step}) behaviors under standard conditions. We note that Corollary \ref{coro:alg1_conv_rate_const_step} provides  one of the first constant learning rate results in reinforcement learning. In { \S\ref{sec:conv_second_stationary_point}}, we  focus on problems with positive bounded rewards and policies whose parameterizations are \emph{regular}, and propose a variant of policy gradient method that employs a periodically enlarged stepsize scheme.
 The salient feature of this modified algorithm is that it is able to escape saddle points, an undesirable subset of stationary points, and converge to second-order stationary points (Theorem \ref{thm:conv_MRPG}). Numerical experiments in  \S\ref{sec:simulations} corroborate our main findings: for Algorithm \ref{alg:RPG}, the use of random rollout horizons avoids stochastic gradient bias and hence exhibits reliable convergence that matches the theoretically established rates; moreover, for the {modified RPG algorithm}, use of periodically enlarged stepsizes makes it possible to escape   from undesirable saddle points and yields   better limiting solutions. All proofs, which constitute an integral part of the paper, are relegated to nine appendices at the end of the paper, so as not to disrupt the flow of the presentation of the main results. 
 
% \kznote{We may need to discuss and agree on some of the terms used in the Introduction, as well as throughout the paper.}


\vspace{6pt}
\noindent \textbf{Notations:} We denote the probability distribution over the space $\cS$ by $\cP(\cS)$, and the  set of integers $\{1,\cdots,N\}$ by $[N]$. We  use $\RR$ to denote the set of real numbers, and $\EE$ to denote the expectation operator. We let $\|\cdot\|$  denote the $2$-norm of a vector in $\RR^d$, or the  spectral norm of a matrix in $\RR^{d\times d}$. We  use $|\cA|$ to denote the cardinality of a finite set $\cA$, or the area of a  region $\cA$, i.e., $|\cA|=\int_{\cA}da$. For any matrix $A\in\RR^{d\times d}$, we use $A\succ 0$ and $A\succeq 0$ to denote that $A$ is positive definite and positive semi-definite, respectively.  We  use $\lambda_{\min}(A)$ and $\lambda_{\max}(A)$ to denote, respectively, the smallest and largest eigenvalues of some square symmetric matrix  $A$, respectively. We use $\EE_X$ or $\EE_{X\sim f(x)}$ to denote the expectation with respect to random variable $X$. Otherwise specified, we   use $\EE$ to denote the full expectation with respect to all random variables.  





==> my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}


